Video Quality Assessment: A Comprehensive Survey

Video quality assessment (VQA) is an important processing task, aiming at predicting the quality of videos in a manner highly consistent with human judgments of perceived quality. Traditional VQA models based on natural image and/or video statistics, which are inspired both by models of projected images of the real world and by dual models of the human visual system, deliver only limited prediction performances on real-world user-generated content (UGC), as exemplified in recent large-scale VQA databases containing large numbers of diverse video contents crawled from the web. Fortunately, recent advances in deep neural networks and Large Multimodality Models (LMMs) have enabled significant progress in solving this problem, yielding better results than prior handcrafted models. Numerous deep learning-based VQA models have been developed, with progress in this direction driven by the creation of content-diverse, large-scale human-labeled databases that supply ground truth psychometric video quality data. Here, we present a comprehensive survey of recent progress in the development of VQA algorithms and the benchmarking studies and databases that make them possible. We also analyze open research directions on study design and VQA algorithm architectures. Github link: https://github.com/taco-group/Video-Quality-Assessment-A-Comprehensive-Survey.

==> sections/7_challenge.tex <==
\section{Current Challenges and Future Work}
\label{future_work}
% Although paramount progress has been made in the deep learning algorithms for video quality assessment, there remains a variety of challenges for researchers to tackle in the future work. In this section, we summarize and discuss the main challenges and opportunities.
Although deep learning algorithms have greatly advanced video quality assessment, numerous challenges remain for future research.
%
In this section, we outline and discuss key challenges and potential opportunities in this field.

\subsection{Datasets}
\label{future_dataset}

Most existing video quality assessment datasets are small, which limits their usefulness in unlocking the potential of data-driven deep learning of visual quality.
%
Unlike mainstream computer vision tasks, like classification and object detection, constructing large-scale, unbiased datasets for VQA problems is quite time-consuming and labor-intensive.
%
This is largely due to the need for increasingly accurate data collection methodolgies and for increased human subjective involvement in psychometric studies of video quality.


Video quality datasets, at least in the aggregate sense, also need to be diverse enough to meet the high demands and popularity of streaming videos consumed by billions worldwide.
%
They also need to be representative of the many different existing, emerging, and future video formats, representations, and display technologies.
%
Given the rapid development of user video devices and streaming media technologies, many advanced video formats such as high framerate (HFR)\cite{madhusudana2021st}, \cite{9497087}, \cite{zheng2022faver}, high dynamic range (HDR)\cite{ebenezer2024hdr,10325414,ebenezer2023making} high resolution (HR), and virtual/extended reality (VR/XR) are becoming widely available.
%
A variety of video content, such as screen content, user-generated content (UGC), professionally generated content (PGC), AI-generated content (AIGC), telepresence content, point cloud data, and augmented/virtual reality (AR/VR) sources, are viewed and evaluated both online and offline daily.
%
There will undoubtedly be a growing need for perceptual quality assessment of constantly expanding types of videos in the future, if only because each evolution generally requires more data.


\subsection{Model Architectures}
\label{model}

Pre-trained neural networks that are widely used for high-level computer vision tasks, such as image classification, have demonstrated their ability to extract quality-aware spatial features.
%
However, video quality assessment is largely a low-level task, focusing on evaluating information degradation of high-quality sources. 
%
Therefore, there is a need to conduct a systematic analysis, to achieve an understanding of how the layers and blocks of successful deep VQA architectures function.
%
Based on this analysis, bespoke deep learning architectures could be specifically developed for visual quality assessment tasks, allowing for the better learning of deep, distortion-aware models that could guide every aspect of video content creation, processing, delivery, and display.

Previous research has often attempted to apply increasingly comprehensive psychovisual and neuroscience theories to the design of algorithms and architectures for VQA, focusing on concepts such as visual saliency~\cite{zhang2014vsi,shi2017perceptual,ortiz2014full,xu2021perceptual,varga2022no}, memory effects~\cite{kim2018deep,li2022study,li2019quality,20219506420,telili20222bivqa}, and perceptual straightening~
\cite{kancharla2021completely,henaff2019perceptual,9921340}.
%
To achieve better predictions of human visual experience, it will be necessary to incorporate increasingly detailed models of the function of visual awareness, and visual behavior.

Current research using large models for IQA and VQA has explored two primary methods: prompt-driven assessment~\cite{wu2023q,Wang_Chan_Loy_2023,wu2023exploringopinionunawarevideoquality,wu2023towards,10448422,wu2023qalign,ge2024lmm} and feature-based assessment~\cite{Yuan_2024_CVPR,He_2024_CVPR,Lu_2024_CVPR,Wen_2024_CVPR,li2023sam,li2023samscore}. 
%
Prompt-driven assessment leverages structured prompts to extract quality judgments directly from large models, making it simple and adaptable. 
%
Feature-based assessment, on the other hand, focuses on extracting visual quality features from pre-trained large models and applying regression techniques to predict quality scores.
%
However, challenges remain in both approaches. 
%
For prompt-driven evaluation, aligning model outputs with precise human-like quality scores is difficult due to the inherent ambiguity in textual responses. 
%
Feature-based assessment, on the other hand, faces issues in ensuring that the extracted features are optimally suited to capture distortions, especially in dynamic video content.
%
Future work should focus on improving the interpretability and consistency of large models’ outputs. 
%
Additionally, developing more efficient architectures for feature extraction and refining prompt design will be crucial to better leverage the power of LLMs and LMMs in IQA and VQA tasks.

While most VQA research has aimed to maximize quality prediction accuracy, the computational complexity of VQA models has been less well-studied, even though it is of considerable practical consequence.
%
However, some recent models, such as RAPIQUE~\cite{tu2021rapique}, FAST-VQA~\cite{wu2022fast} and Faster-VQA~\cite{10264158} have been designed to be both accurate and highly efficient.
%
Still, there remains significant room (and demand) for the development of highly efficient, reliable VQA models both in the application space, as well as in training complexity.

\subsection{Training Techniques}
\label{training_method}

The limitations imposed by the continuing (but improving) shortfall of adequate ground-truth human subjective data of visual quality have been long-standing, making effective VQA network training a more significant challenge.
%
Various solutions have been proposed to enrich datasets, including training on patches or clips that share labels with the same images/videos derive from, or using proxy scores from reliable quality models, like VMAF as sources of pseudo ground truth.
%
Some recent studies have shown that it is possible to train powerful VQA network without any subjective scores, by using other kinds of non-human-labeled data, such as large numbers of videos having precisely known distortions, and by the use of contrastive learning~\cite{madhusudana2022image,madhusudana2022conviqt} or other unsupervised learning protocols~\cite{saha2023re}.

The selection of a suitable loss function is another crucial aspect when training deep VQA models.
%
A reliable loss function should enable a model to produce accurate, consistent quality predictions and be both computationally efficient and easy to optimize.
%
Evidently, the nature of the task is a primary determinant in loss function selection. For instance, binary or categorical cross-entropy loss is suitable for predicting video distortion types, while MSE/MAE are optimal for continuous quality score prediction, and contrastive loss can learn similarity metrics between pairs of videos.
%
Furthermore, given the finite ranges of predictable values learned and delivered by VQA models, unbounded loss functions like MSE/MAE can over-penalize discrepancies between predicted and ground-truth quality scores in challenging scenarios.
%
In such cases, choosing a compound loss function, or a variant of MSE/MAE, like Huber loss, could be beneficial.

